Mediating Human-Swarm Interactions Through a Robot Helper: A Shepherding-Inspired Approach

This work investigates human-swarm interaction (HSI) for steering large collectives through an intermediary robot helper. While prior robot-swarm control and HSI techniques commonly assume swarm members are addressable, these assumptions often fail for ``ungovernable'' swarms such as wildlife flocks and schools of fish. Motivated by pastoral shepherding, we compare low-level teleoperation to a higher-autonomy motion-primitives interface in a virtual reality (VR) shepherding task under varied swarm cohesion dynamics. Results indicate that motion primitives that operate on collective shape (e.g., boundary-based control) improve task performance and reduce perceived workload.

==> results_backup.tex <==
\section{RESULTS}

\subsection{Task Performance}
The primary quantitative performance metric was the number of boids successfully guided into the holding pen by the end of each trial. As described in Section~3.3, each trial began with 25 boids. Participants were instructed to herd as many boids as possible into the pen within the allotted time; each particle that entered the pen contributed one point. The final score therefore served as the operational measure of task performance. Figure~2 presents aggregated performance across all conditions.

To test for effects of interface and swarm dynamics, performance was analyzed using a $2\times2$ repeated-measures ANOVA (Interface: Teleoperation vs.\ Shepherding; Cohesion: Low vs.\ High). The analysis showed a strong main effect of Interface, $F(1,19)=62.09$, $p<.001$, and a strong main effect of Cohesion, $F(1,19)=77.21$, $p<.001$, with no significant Interface$\times$Cohesion interaction, $F(1,19)=2.47$, $p=0.133$.

Overall, Figure~2 shows a clear separation between interfaces: participants achieved higher scores under shepherding than teleoperation. Teleoperation performance also differed noticeably between low- and high-cohesion swarms, suggesting that users had to adapt low-level control strategies to changes in swarm stability. In contrast, performance under shepherding was comparatively consistent across cohesion levels, which aligns with the design intent of the motion primitives: hull-based flanking and driving behaviors are defined relative to the swarm geometry and thus generalize more readily across swarm configurations than manual teleoperation. 



\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{combined_performance_violin_8_6.png}
    \caption{Task Performance Results}
    \label{fig:placeholder}
\end{figure}


\subsection{Subjective Workload}
Following each trial, participants completed the NASA Task Load Index (NASA-TLX) to assess subjective workload. NASA-TLX conceptualizes workload as a multidimensional construct spanning \emph{Mental Demand}, \emph{Physical Demand}, \emph{Temporal Demand}, \emph{Performance}, \emph{Effort}, and \emph{Frustration} \cite{Hart1988,Hart2006}. We computed an overall workload score as the mean of the six subscales:

\begin{equation}
\text{NASA-TLX}_{\text{overall}} = \frac{1}{6} \sum_{i=1}^{6} S_i,
\end{equation}

where $S_i$ denotes each subscale score. Figure~3 summarizes NASA-TLX workload across conditions.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{combined_workload_violin (1).png}
    \caption{NASA-TLX Results}
    \label{fig:workload}
\end{figure}

Workload was analyzed using a $2\times2$ Repeated-Measures ANOVA (Interface: Teleoperation vs.\ Shepherding; Cohesion: Low vs.\ High). The analysis showed a significant main effect of Interface, $F(1,19)=26.29$, $p<.001$, indicating lower workload under shepherding, while Cohesion and the Interface$\times$Cohesion interaction were not significant.

Overall, Figure~3 suggests that the shepherding interface reduces subjective workload, but the separation is smaller than for task performance. This is plausible because NASA-TLX aggregates multiple components of workload: autonomy-related benefits may primarily reduce \emph{Mental Demand} and \emph{Effort}, whereas other dimensions (e.g., \emph{Temporal Demand}) remain similar because both conditions impose identical time limits and comparable task pacing \cite{Hart1988}. In addition, even with motion primitives, participants must maintain situation awareness (e.g., monitoring flock shape and timing command switches), which can preserve workload despite reduced low-level control requirements \cite{Hart2006,Beer2014}. Finally, short, game-like trials can compress subjective ratings, making moderate differences harder to detect even when objective performance diverges \cite{Hart2006}. Together, these factors help explain why autonomy produces clearer gains in performance than in overall perceived workload.


\subsection{\textbf{Open-Ended Reflections}}
Findings from the semi-structured interview questions shed light on how the two conditions were perceived. The first author extracted interesting insights and snippets from the interviews conducted across participants. 

\subsubsection{Preference for Condition}
Out of all participants, there was a leaning towards using the shepherding commands condition, but only sightly. Of the 24 participants tested, 14 preferred to use the shepherding commands, with the remaining 10 preferring to use the teleoperation commands. The primary differentiating factor for the two conditions is the amount of control users have over the agent, as well as the mental demand placed on the user during the task. Table 3 contains interview snippets containing comments from participants that emerged during interviews. 

\begin{table}[h]
\caption{Interview Snippets on Preference for Control Condition}
\centering
\setlength{\tabcolsep}{6pt}
\footnotesize
\begin{tabularx}{\linewidth}{>{\raggedright\arraybackslash}p{1cm} >{\raggedright\arraybackslash}X}
\toprule
\textbf{Participant ID} & \textbf{Snippet} \\
\midrule
p3 &
\textbf{When asked about what condition they prefer, and why}: `the teleoperation condition, just because I like to have control over the agent at all times' \\

p10 &
\textbf{When asked about what condition they prefer, and why}: `the shepherding condition, because it's easier on the shepherd and harder on the sheepdog' \\

p12 &
\textbf{When asked about what condition they prefer, and why}: `the first (shepherding) condition; it seemed like the dog knew exactly what to do, and when I controlled the dog, I kept messing up' \\

% p16 &
% \textbf{When asked about what condition they prefer, and why}: `i like the convenience of the shepherding condition, but I prefer having control over the agent when the group splits. With the shepherding condition, it felt like the agent was confused sometimes' \\

% p20 &
% \textbf{When asked about what condition they prefer, and why}: `i prefer the first (shepherding) condition as it felt like I had a partner to help me with the task, it was very well made' \\
\bottomrule
\end{tabularx}
\end{table}



\subsubsection{Swarm Dynamics}
In most cases (17/24), participants were also able to accurately point out that there was a difference in the swarm behavior between trials. In many cases however, participants blamed themselves for observing the difference in the between the conditions. This is further illustrated by the snippets supporting this section  

\begin{table}[h]
\caption{Interview Snippets on Swarm Dynamics}
\centering
\setlength{\tabcolsep}{6pt}
\footnotesize
\begin{tabularx}{\linewidth}{>{\raggedright\arraybackslash}p{1cm} >{\raggedright\arraybackslash}X}
\toprule
\textbf{Participant ID} & \textbf{Snippet} \\
\midrule
p5 &
\textbf{When asked if they observed any difference in the swarm between different trials}: `yes, I feel like the swarm was more obedient in this case as they stayed together better than the previous trial' \\

% p7 &
% \textbf{When asked if they observed any difference in the swarm between different trials}: `it felt like the boids had a mind of their own in this trial. I tried to round up the group, but they just didn't want to be together' \\

p11 &
\textbf{When asked if they observed any difference in the swarm between different trials}: `the swarm split up very early, and I don't know if this was because of the strategy I employed, or because the group did not want to stay together' \\

% p17 &
% \textbf{When asked if they observed any difference in the swarm between different trials}: `it really felt like this swarm was more cohesive in this trial, it was so easy to work with' \\
\bottomrule
\end{tabularx}
\end{table}


\subsubsection{Cognitive Load}
Participants reported that the lower-autonomy teleoperation condition afforded finer-grained control over the helper agent, but required sustained attention to trajectory planning, spatial positioning, and continuous motion regulation. In contrast, the motion-primitives condition reduced the need for moment-to-moment control decisions. 

These subjective accounts align with the quantitative workload findings and are illustrated through representative interview excerpts presented in Table 5.


\begin{table}[h]
\caption{Interview Snippets on Cognitive Load}
\centering
\setlength{\tabcolsep}{6pt}
\footnotesize
\begin{tabularx}{\linewidth}{>{\raggedright\arraybackslash}p{1cm} >{\raggedright\arraybackslash}X}
\toprule
\textbf{Participant ID} & \textbf{Snippet} \\
\midrule
% p6 &
% \textbf{When asked to describe how the trial went}: `(for the shepherding condition) it went great! It was almost as if the agent knew the best way to move the swarm' \\

p9 &
\textbf{When asked to describe how the trial went}: `(for the teleoperation condition) i really enjoyed it though I could not get all of them in. I think I might have to change my strategy for the next trial and try to round up the swarm before' \\

p15 &
\textbf{When asked about how demanding the two trials were compared to each other}: `in the first condition (teleoperation), I felt like I was responsible for the dog's movement at all times and I couldn't take a break. the second condition was easier because i was more relaxed' \\

% p19 &
% \textbf{When asked about how easy or difficult was it to learn the control scheme for both conditions}: `it was definitely easier for the second condition (teleoperation) since I have played video games in the past where the character is controlled by the joystick, but the first condition (shepherding) was also not that hard' \\
\bottomrule
\end{tabularx}
\end{table}



\subsubsection{Novel Control Schemes}
As part of the post-trial assessment, participants were invited to propose an ideal control scheme after having experienced both interaction conditions. This open-ended prompt was intended to elicit reflections on interface preferences and perceived trade-offs.

A majority of participants (14/24) suggested a hybrid approach that combined elements of continuous teleoperation with discrete motion primitives. A smaller subset indicated satisfaction with the shepherding-based motion-primitives condition as implemented. Additionally, a few participants proposed novel control strategies that were not represented in either experimental condition.

Representative excerpts illustrating these perspectives are presented in~\ref{Table 6}.



% \begin{table}[h]
% \caption{Interview Snippets on Control Schemes}
% \centering
% \setlength{\tabcolsep}{6pt}
% \footnotesize
% \begin{tabularx}{\linewidth}{r l X}
% \toprule
% \textbf{S. No.} & \textbf{Participant ID} & \textbf{Snippet} \\
% \midrule
% 1 & p5 
%   & \textbf{When asked what their ideal control scheme for this task would be}: 'I like the sheepdog control scheme, but the arcs the dog made around the swarm were too tight sometimes. I would like for there to be an additional button that helps me fine-tune the arc radius' \\

% 2 & p8 
%   & \textbf{When asked what their ideal control scheme for this task would be}: 'the agent had a mind of its own sometimes and I would like to have the ability to point it towards the group I want to herd in case of splits'  \\

% 3 & p13 
%   & \textbf{When asked what changes they would make to the agent to make the task easier}: 'I think having multiple helpers instead of a single helper would be good, because I can then send helpers to round up split groups' \\
  
% \bottomrule
% \end{tabularx}
% \end{table}

\begin{table}[h]
\caption{Interview Snippets on Control Schemes}
\centering
\setlength{\tabcolsep}{6pt}
\footnotesize
\begin{tabularx}{\linewidth}{>{\raggedright\arraybackslash}p{1cm} >{\raggedright\arraybackslash}X}
\toprule
\textbf{Participant ID} & \textbf{Snippet} \\
\midrule
p5 &
\textbf{When asked what their ideal control scheme for this task would be}: `I like the sheepdog control scheme, but the arcs the dog made around the swarm were too tight sometimes. I would like for there to be an additional button that helps me fine-tune the arc radius' \\

% p8 &
% \textbf{When asked what their ideal control scheme for this task would be}: `the agent had a mind of its own sometimes and I would like to have the ability to point it towards the group I want to herd in case of splits' \\

p13 &
\textbf{When asked what changes they would make to the agent to make the task easier}: `I think having multiple helpers instead of a single helper would be good, because I can then send helpers to round up split groups' \\
\bottomrule
\end{tabularx}
\end{table}




\label{sec:RESULTS}

